SplineGS: Robust Motion-Adaptive Spline for Real-Time Dynamic 3D Gaussians from Monocular Video

Synthesizing novel views from in-the-wild monocular videos is challenging due to scene dynamics and the lack of multi-view cues. To address this, we propose SplineGS, a COLMAP-free dynamic 3D Gaussian Splatting (3DGS) framework for high-quality reconstruction and fast rendering from monocular videos. At its core is a novel Motion-Adaptive Spline (MAS) method, which represents continuous dynamic 3D Gaussian trajectories using cubic Hermite splines with a small number of control points. For MAS, we introduce a Motion-Adaptive Control points Pruning (MACP) method to model the deformation of each dynamic 3D Gaussian across varying motions, progressively pruning control points while maintaining dynamic modeling integrity. Additionally, we present a joint optimization strategy for camera parameter estimation and 3D Gaussian attributes, leveraging photometric and geometric consistency. This eliminates the need for Structure-from-Motion preprocessing and enhances SplineGS's robustness in real-world conditions. Experiments show that SplineGS significantly outperforms state-of-the-art methods in novel view synthesis quality for dynamic scenes from monocular videos, achieving thousands times faster rendering speed.

==> table/iphone_quantitative.tex <==
\begin{table*}[t]
\label{table:iphone_quantitative}
\vspace{-0.5cm}
\begin{center}
\setlength\tabcolsep{6pt} % default value: 6pt
\renewcommand{\arraystretch}{1.1}
\scalebox{0.7}{
\begin{tabular}{ c | c | c c c c c c c | c }
\toprule
& Method & Apple & Block & Paper-windmill & Space-out & Spin & Teddy & Wheel & \textbf{Average} \\  
\bottomrule
\hline\noalign{\smallskip}
\multirow{6}{*}{COLMAP} &STGS~\cite{Li_STG_2024_CVPR}       & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&D3DGS~\cite{yang2023deformable3dgs}   & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&4DGS~\cite{Wu_2024_CVPR} & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&RodynRF~\cite{liu2023robust}       & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&DynNeRF~\cite{Gao-ICCV-DynNeRF} & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&MonoNeRF~\cite{23iccv/tian_mononerf}   & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
\midrule
\multirow{3}{*}{COLMAP-Free} & RodynRF~\cite{liu2023robust}        & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&MoSca~\cite{lei2024moscadynamicgaussianfusion}        & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
&\textbf{SplineGS (Ours)} & 25.66 / 0.071 & 28.68 / 0.040 & 29.13 / 0.063 & 24.26 / 0.089 & 22.37 / 0.103 & 26.19 / 0.054 & 24.96 / 0.048 & 25.89 / 0.067  \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}
